Molecular Design Based on Artificial Neural Networks, Integer Programming and Grid Neighbor Search

A novel framework has recently been proposed for designing the molecular structure of chemical compounds with a desired chemical property using both artificial neural networks and mixed integer linear programming. In the framework, a chemical graph with a target chemical value is inferred as a feasible solution of a mixed integer linear program that represents a prediction function and other requirements on the structure of graphs. In this paper, we propose a procedure for generating other feasible solutions of the mixed integer linear program by searching the neighbor of output chemical graph in a search space. The procedure is combined in the framework as a new building block. The results of our computational experiments suggest that the proposed method can generate an additional number of new chemical graphs with up to 50 non-hydrogen atoms.

==> Result_2LMM_ANN_grid_Phase2_temp.tex <==

\medskip \noindent
{\bf Results on Phase~2.  }
To execute  Stages~4  and 5 in Phase~2, 
we used a set of seven instances
$I_{\mathrm{a}}$, $I_{\mathrm{b}}^i, i\in[1,4]$, $I_{\mathrm{c}}$
 and $I_{\mathrm{d}}$ based on the seed graphs prepared by Zhu et~al.~\cite{ZAHZNA21}. 
We here present their seed graphs $\GC$ 
(see Appendix~\ref{sec:specification} for the details of $I_{\mathrm{a}}$
and Appendix~\ref{sec:test_instances} for the details of 
$I_{\mathrm{b}}^i, i\in[1,4]$, $I_{\mathrm{c}}$  and $I_{\mathrm{d}}$).

The seed graph  $\GC$ of  $I_{\mathrm{a}}$ is given
 by the graph in Figure~\ref{fig:specification_example_1}(a).
The seed graph $\GC^1$ of  $I_{\mathrm{b}}^1$
(resp., $\GC^i, i=2,3,4$ of $I_{\mathrm{b}}^i,  i=2,3,4$) is illustrated
 in Figure~\ref{fig:specification_example_polymer}.
 
\begin{figure}[h!] \begin{center}
\includegraphics[width=.85\columnwidth]{fig/specification_example_polymer.eps}
\end{center} \caption{%An illustration of seed graphs:
%  for inferring cyclic graphs with rank at most 2: 
(i)  Seed graph   $\GC^1$ for $I_{\mathrm{b}}^1$ and  $I_{\mathrm{d}}$;
(ii) Seed graph $\GC^2$   for $I_{\mathrm{b}}^2$; 
(iii) Seed graph  $\GC^3$   for $I_{\mathrm{b}}^3$; 
(iv)  Seed graph $\GC^4$  for $I_{\mathrm{b}}^4$. }
\label{fig:specification_example_polymer}
\end{figure} 

Instance  $I_{\mathrm{c}}$ has been introduced 
in order to infer a chemical graph $\Co^\dagger$ such that
the core of $\Co^\dagger$ is equal to the core of 
chemical graph $\Co_A$: CID~24822711 in Figure~\ref{fig:instance_I_c_I_d}(a)
and 
the frequency of each edge-configuration in the non-core of $\Co^\dagger$
is equal to that of chemical graph  $\Co_B$:  CID~59170444
 in  Figure~\ref{fig:instance_I_c_I_d}(b).
This means that the seed graph  $\GC$ of   $I_{\mathrm{c}}$
 is the core of $\Co_A$
which is indicated by a shaded area in  Figure~\ref{fig:instance_I_c_I_d}(a). 

Instance  $I_{\mathrm{d}}$ has been introduced 
in order to   infer a chemical monocyclic graph $\Co^\dagger$ such that
the frequency vector of  edge-configurations in  $\Co^\dagger$
is a vector obtained by merging those of chemical graphs 
$\Co_A$: CID~10076784   and $\Co_B$: CID~44340250 
in   Figure~\ref{fig:instance_I_c_I_d}(c) and (d), respectively.  
The seed graph  $\GC$ of    $I_{\mathrm{d}}$  is given by  $\GC^1$  
 in Figure~\ref{fig:specification_example_polymer}(i).

\begin{figure}[!htb]
\begin{center} 
 \includegraphics[width=.69\columnwidth]{fig/instance_I_c_I_d.eps}
\end{center}
\caption{An illustration of  chemical compounds 
  for instances  $I_{\rm c}$  and  $I_{\rm d}$: 
(a) $\Co_A$: CID~24822711;
(b)  $\Co_B$: CID~59170444; 
(c) $\Co_A$: CID~10076784;
(d)  $\Co_B$: CID~44340250,
where hydrogens are omitted. 
}
\label{fig:instance_I_c_I_d}  
\end{figure}  


\medskip \noindent
{\bf Stage~4.  } 
We executed Stage~4 for three properties $\pi\in \{${\sc FP,  OptR,  SfT}$\}$.  

 For the MILP formulation  $\mathcal{M}(x,y;\mathcal{C}_1)$,
we use the prediction function  
 that attained the median  test $\mathrm{R}^2$ in Table~\ref{table:phase1b}.
 To solve an MILP   in Stage~4, we used % CPLEX~\cite{cplex}.
{\tt  CPLEX} version 12.10.
Tables~\ref{table:stages_4_5_Fp} and \ref{table:stages_4_5_SfT}  show
   the computational results of the experiment
in Stage~4 for the five properties, 
 where we denote the following:
\begin{enumerate} [nosep,  leftmargin=*]
  
\item[-]  
$n_\LB$: a lower bound on the number of non-hydrogen atoms 
in  a chemical graph $\Co$ to be inferred; 

\item[-]  
  $ \underline{y}^*,~\overline{y}^* $:  
 lower and upper bounds $\underline{y}^*, \overline{y}^*\in \R$ 
  on the value $a(\Co)$ of a chemical graph $\Co$ to be inferred; 
  
\item[-]  
 $\#$v (resp.,  $\#$c): 
 the number  of variables (resp., constraints)  in the MILP  in Stage~4;  
  
\item[-]   
 I-time: the   time (sec.) to solve the MILP  in Stage~4; 

\item[-]  
    $n$:  the number  $n(\Co^\dagger)$  of  non-hydrogen atoms
     in the chemical graph $\Co^\dagger$   inferred in Stage~4;   
     
\item[-]  
  $\nint$:  the number  $\nint(\Co^\dagger)$ of interior-vertices in
  the chemical graph $\Co^\dagger$   inferred in Stage~4; and 
      
\item[-]  
$\eta$: the predicted property value 
$\eta(f(\Co^\dagger))$ of the chemical graph $\Co^\dagger$ inferred 
in Stage~4.
\end{enumerate}


  
\begin{table}[h!]\caption{ Results of Stages~4 and 5 for  {\sc Fp}.}  
 \begin{center}
 \begin{tabular}{@{}  c  c   c  r r r r r c  r r r     @{}}\hline                
 inst. & $n_\LB$ &  $ \underline{y}^*,~\overline{y}^* $ & $\#$v~  &  $\#$c~~   &  
   {\small I-time}\!\! & $n$~  &  \!\!$\nint$  &  $\eta $ \!\! & 
                 {\small  D-time} &  {\small $\Co$-LB} &  {\small $\#\Co$}    \\ \hline
   $I_{\mathrm{a}}$ & 30 &  130,\,133 &10877 &10604& 13.7 &42 &25 &132.827 &0.0703& 1 &1   \\%
  $I_{\mathrm{b}}^1$ & 10 & 110,\,113 &10773 & 8255 &2.00 &10 & 7 &112.428 &0.0234 & 2 &2  \\%
  $I_{\mathrm{b}}^2$ & 20 &  215,\,218 &13217 &11366 &44.1&49 &25 &217.597 &0.594&   $1.9\mathrm{E}4$ &100 \\%
  $I_{\mathrm{b}}^3$ & 30 &  110,\,113 &12993 &11346 &43.6 &48 &30& 110.193& 17.2&  $2.4\mathrm{E}7$& 100  \\%
  $I_{\mathrm{b}}^4$ & 40 &  137,\,140 &12767& 11324 &148.0&44 &25& 138.116 &0.16 &948 &100  \\%
  $I_{\mathrm{c}}$   & 40 &  150,\,153& 7900& 8629& 4.38  &50 &34& 151.133& 0.0197 &1 &1  \\%
  $I_{\mathrm{d}}$   & 40 &  -63,\,-61& 6507& 8106& 33.2  &45& 23& -61.733 &251.0 &  $4.9\mathrm{E}9$ &100  \\% \\
   \hline
   \end{tabular}\end{center}\label{table:stages_4_5_Fp}
\end{table}
Figure~\ref{fig:MILP_solutions}(a) illustrates  the chemical graph  $\Co^\dagger$  inferred 
 from   $I_{\mathrm{a}}$  with $(\underline{y}^*, \overline{y}^*) =(130,133)$  of  {\sc Fp}
  in Table~\ref{table:stages_4_5_Fp}.   
  
 
 \begin{table}[h!]\caption{ Results of Stages~4 and 5 for {\sc OptR}.}  
 \begin{center}
 \begin{tabular}{@{}  c  c   c  r r r r r c  r r r     @{}}\hline                
 inst. & $n_\LB$ & $ \underline{y}^*,~\overline{y}^* $ & $\#$v~  &  $\#$c~~   &  
   {\small I-time}\!\! & $n$~  &  \!\!$\nint$  &   $\eta$   & 
                 {\small  D-time} &  {\small $\Co$-LB} &  {\small $\#\Co$}    \\ \hline 
   $I_{\mathrm{a}}$ & 30 &  81,\,83  & 10036 & 10396  & 4.32  & 47 & 26 & 81.587  & 0.066  & 2  & 2        \\%
  $I_{\mathrm{b}}^1$ & 10 &   -78,\,-76  &10570  & 8128 & 104.0 & 19  & 15 & -78.0 & 0.176 & 60 & 60      \\%
  $I_{\mathrm{b}}^2$ & 20 &   50,\,52  &12952  & 11231 & 41.2  & 49  &25 & 51.452  & 0.21 & 1616 & 100    \\%
  $I_{\mathrm{b}}^3$ & 30 &  30,\,32  &12722  &11201  & 37.3  &50  &25 & 31.261 & 0.186  &210  &100  \\%
  $I_{\mathrm{b}}^4$ & 40 &  116,\,118 & 12491 & 11171 & 17.7  & 49  &25  &117.918 & 0.883  &$3.7\mathrm{E}4$ & 100   \\%
  $I_{\mathrm{c}}$   & 40 &   -30,\,-28  &7885 & 8493  & 4.84  &49 & 33 & -29.163  &0.0159 & 1 & 1     \\%
  $I_{\mathrm{d}}$   & 40 &   40,\,42  &6495 &7976  & 10.5   &40 & 23 & 40.152 & 2.52 & $7.3\mathrm{E}5$ & 100  \\% \\
   \hline
   \end{tabular}\end{center}\label{table:stages_4_5_OptR}
\end{table}
 Figure~\ref{fig:MILP_solutions}(b) illustrates  the chemical graph  $\Co^\dagger$  inferred
 from   $I_{\mathrm{b}}^2$ with $(\underline{y}^*, \overline{y}^*) =(50, 52)$   of  {\sc OptR}
  in Table~\ref{table:stages_4_5_OptR}. 
  
 
 \begin{table}[h!]\caption{ Results of Stages~4 and 5 for {\sc SfT}.}  
 \begin{center}
 \begin{tabular}{@{}  c  c  c  r r r r r c  r r r     @{}}\hline                
 inst. &  $n_\LB$ &  $ \underline{y}^*,~\overline{y}^* $ & $\#$v~  &  $\#$c~~   &  
   {\small I-time}\!\! & $n$~  &  \!\!$\nint$  & $\eta$   & 
                 {\small  D-time} &  {\small $\Co$-LB} &  {\small $\#\Co$}    \\ \hline
   $I_{\mathrm{a}}$ & 30 &   40,\,41 & 9288  &10207  &2.10  &41 & 22 & 40.231  &0.0638  &1  &1   \\%
  $I_{\mathrm{b}}^1$ & 10 &  28,\,29 & 7965 & 7599  &2.28 & 11 & 5  &28.488 & 0.00927  &1  &1   \\%
  $I_{\mathrm{b}}^2$ & 20 &  42,\,43  &9583  &10719 & 12.0  &48 & 25 & 42.998  &0.163  &200 & 100     \\%
  $I_{\mathrm{b}}^3$ & 30 & 36,\,37  &9326 & 10700 & 9.87  &42 & 25 & 36.358 & 9.39  &$9.2\mathrm{E}4$ & 100   \\%
  $I_{\mathrm{b}}^4$ & 40 & 43,\,44  &9069 & 10682  &13.4  &46 & 25 & 43.857  &0.123 & 116 & 100    \\%
  $I_{\mathrm{c}}$   & 40 &  44,\,45 & 7777 & 8378 & 4.37 & 45  &32 & 44.557  &0.0158 & 1  &1  \\%
  $I_{\mathrm{d}}$   & 40 &  39,\,40  &6385  &7857 & 6.72  &44 & 23  &39.55  &29.9 &  $2.8\mathrm{E}7$ &100  \\% \\
   \hline
   \end{tabular}\end{center}\label{table:stages_4_5_SfT}
\end{table}
Figure~\ref{fig:MILP_solutions}(c) illustrates  the chemical graph  $\Co^\dagger$  inferred 
 from  $I_{\mathrm{c}}$ with $(\underline{y}^*, \overline{y}^*) =(44, 45)$  of  {\sc  SfT}
  in Table~\ref{table:stages_4_5_SfT}.   
 
 
\begin{figure}[!htb]
\begin{center} 
\includegraphics[width=.98\columnwidth]{fig/MILP_solutions.eps}
\end{center}
\caption{ 
(a)  $\Co^\dagger$ with   $\eta(f(\Co^\dagger))= 132.827$ inferred
  from   $I_{\mathrm{a}}$ with $(\underline{y}^*, \overline{y}^*) =(137,\,140 )$  of  {\sc Fp};  
  %  
(b)  $\Co^\dagger$ with   $\eta(f(\Co^\dagger))=51.452$ inferred
 from   $I_{\mathrm{b}}^2$ with $(\underline{y}^*, \overline{y}^*) =(50, 52)$  of  {\sc OptR}; and   
 %
(c)  $\Co^\dagger$ with  
  $\eta(f(\Co^\dagger))=44.557$ inferred
  from   $I_{\mathrm{c}}$ with $(\underline{y}^*, \overline{y}^*) =(44, 45)$  of  {\sc SfT}.   
}
\label{fig:MILP_solutions}  
\end{figure}  
 
In this experiment, we prepared several different types of instances:
 instances  $I_{\mathrm{a}}$ and $I_{\mathrm{c}}$ have restricted seed graphs,
the other  instances  have abstract seed graphs and
instances $I_{\mathrm{c}}$ and $I_{\mathrm{d}}$ have restricted set of fringe-trees.
From Tables~\ref{table:stages_4_5_Fp} and \ref{table:stages_4_5_SfT},
we observe that an instance with a large number of variables and constraints 
takes more running time than those with a smaller size in general.
All instances in this experiment are solved in a few seconds to around 150 seconds
with our MILP formulation. 

%\input additional_experiment_Stage_4.tex

\medskip \noindent
{\bf Stage~5.  } 
We executed Stage~5 to generate a more number of target chemical graphs $\Co^*$,
where we call a chemical graph $\Co^*$ a {\em chemical isomer} of
a target chemical graph $\Co^\dagger$ of a topological specification $\sigma$
if $f(\Co^*)=f(\Co^\dagger)$ and $\Co^*$ also satisfies the same topological specification $\sigma$.
We computed  chemical isomers  $\Co^*$ of 
each target chemical graph  $\Co^\dagger$ inferred in Stage~4.
We execute an  algorithm for generating chemical isomers of   $\Co^\dagger$
up to 100 when the number of all chemical isomers exceeds 100.
For this, we use a dynamic programming dynamic programming~\cite{ZAHZNA21}. 
The algorithm first decomposes $\Co^\dagger$ into a set of acyclic chemical graphs,
next replace each acyclic chemical graph $T$ with another  acyclic chemical graph $T'$ that admits
the same feature vector as that of $T$
 and finally assemble the resulting acyclic chemical graphs
into a chemical isomer $\Co^*$ of $\Co^\dagger$. 
The algorithm can compute a lower bound 
on the total number of all chemical isomers $\Co^\dagger$
without generating all of them.

Tables~\ref{table:stages_4_5_Fp} and \ref{table:stages_4_5_SfT}  show
   the computational results of the experiment
in Stage~5 for the five properties, 
 where we denote the following:
%
\begin{enumerate}[nosep,  leftmargin=*]
\item[-]
 D-time: the running time (sec.) to execute the dynamic programming algorithm
 in Stage~5 to compute a lower bound on the number 
 of all chemical isomers  $\Co^*$ of  $\Co^\dagger$   
 and generate all (or up to 100) chemical isomers $\Co^*$;
 
\item[-]
 $\Co$-LB: a lower bound on the number of all chemical isomers $\Co^*$ of 
$\C^\dagger$, where $a\mathrm{E}b$ means $a\times 10^{b}$;~and

\item[-]
 $\#\Co$: the number of all (or up to 100) chemical isomers $\Co^*$ of  $\Co^\dagger$  
 generated in Stage~5.
\end{enumerate} 
  
From Tables~\ref{table:stages_4_5_Fp} and \ref{table:stages_4_5_SfT}, we observe  
 the running time and the number of generated isomers  in Stage~5. 
 %

The chemical graph $\Co^\dagger$   in  $I_{\mathrm{b}^3}$
and $I_{\mathrm{d}}$ admits a large number of 
chemical isomers $\Co^*$ in some cases, 
 where a lower bound $\Co$-LB  on the number of chemical isomers
is derived without generating all of them.  
For the other instances, the running time for generating up to 100 target chemical graphs
 in Stage~5 is less than one second.  
 For some chemical graph $\Co^\dagger$, no chemical isomer was found by our algorithm.
 This is because each acyclic chemical graph in the decomposition of $\Co^\dagger$
 has no alternative acyclic chemical graph than the original one. 
 For such an instance, we generate other desired chemical graphs
 by applying our new method of grid neighbor search. 

\medskip \noindent
{\bf Grid Neighbor Search.  } 
As a new building block of the framework of inferring chemical graphs,
we conducted an experiment of applying our grid neighbor search to generate other solutions
of an MILP in Stage~4.
We select the MILP such that a solution $\C^\dagger$ of the MILP 
admits at most two isomers $\C^*$ in Stage~5;
i.e.,    $I_{\mathrm{a}}$ with properties {\sc Fp}, {\sc OptR} and {\sc SfT}; 
$I_{\mathrm{b}}^1$ with properties {\sc Fp}  and {\sc SfT};  and 
$I_{\mathrm{c}}$ with properties {\sc Fp}, {\sc OptR}  and {\sc SfT}.
In this experiment, we set  
 $p_{\max}:=2$, 
 $\delta:=(0.1, 0.1)$, 
 $r:=(3,3)$ and 
 projection functions   $\theta_1$ and $\theta_2$ to be linear prediction functions
  for properties 
solubility ({\sc Sl}) and lipophilicity ({\sc Lp}), respectively,
constructed by Zhu et~al.~\cite{ZAHZNA21}.
The number of non-center grids in the neighbor $N(r)$ is $7\times 7-1=48$,
where the center grid $z=(0,0)$ is always feasible for the selected instances. 
%
For each instance, we check the feasibility of grids  $z \in N(r)$ 
in an non-decreasing order of $\max_{p\in [1,p_{\max}]}|z(p)|$.
For each feasible grid $z \in N(r)$, output a feasible solution $\C^\dagger_z$
of  the augmented MILP instance. 
We set a time limit for checking the feasibility of a grid to be 300 seconds. 
and we skip a grid when the corresponding MILP is not solved within the time limit.
We also discard any grid $z \in N(r)$
without testing the feasibility of $z$ if we find an infeasible grid $z'\in N(r)$
with $z'\prec z$.


Tables~\ref{table:grid}    shows
   the computational results of the experiment
in the grid neighbor search for the eight instances, 
 where we denote the following:
%
\begin{enumerate}[nosep,  leftmargin=*]
\item[-]
instance: a pair $(I,\pi)$ of topological specification $I$ and
a property $\pi$ in the tested instance;

\item[-] $n$: the number of non-hydrogen atoms in the tested instance;  

\item[-] \#feasible:  the number of  non-center grids in $N(r)$
that are found to be feasible during the search procedure; 

\item[-] \#solutions:   the number of chemical graphs
obtained from the feasible non-center grids in $N(r)$,
where the same feasible gird provides two solutions
and \#feasible$>$\#solutions holds in such a case; 

\item[-] \#infeasible: the number of  non-center grids in $N(r)$
that are found to be infeasible during the search procedure; 

\item[-] \#ignored:  the number of  non-center grids $z\in N(r)$
that are ignored due to an infeasible grid $z'z\in N(r)$ with $z'\prec z$
during the search procedure; 

\item[-] \#time  out: the number of  non-center grids in $N(r)$
such that the time for feasibility check exceeds
the time limit of 300 seconds during the search procedure; 

%%%%%%%%%% 
% \item[-] time: the average time for checking the feasibility of
%%% a grid $z\in N(r)$ whose feasibility can be detected within the time limit.
\end{enumerate} 

 \begin{table}[h!]\caption{ Results of Grid Neighbor Search.}  
 \begin{center}
 \begin{tabular}{@{}  c  c c c    c c c c     @{}}\hline            
 instance & $n$ &  \#feasible & \#solutions &  \#infeasible & \#ignored & \#time out & \\ \hline
  $(I_{\mathrm{a}}$,{\sc Fp})   & 42 & 34 & 34  & 0 & 0 & 15 &     \\
  $(I_{\mathrm{a}}$,{\sc OptR}) & 47  & 31 & 31 & 1  & 2 & 15 &   \\
  $(I_{\mathrm{a}}$,{\sc SfT})     & 41 & 46  &  46 & 0 & 0 & ~3 &   \\
  $(I_{\mathrm{b}}^1$,{\sc Fp})     & 10  & 22 &22  & 3  & 3 & 21  & \\
  $(I_{\mathrm{b}}^1$,{\sc SfT})    & 11  &  23 & 23 & 0 & 0 & 26 &    \\
  $(I_{\mathrm{c}}$,{\sc Fp})      &  50 & 34  & 34 & 0 & 0 & 15  &    \\
  $(I_{\mathrm{c}}$,{\sc OptR})     & 49 & 26 & 26 & 1 & 1 & 21 &     \\
  $(I_{\mathrm{c}}$,{\sc SfT})      & 45 & 18 &18  & 3  & 4  & 24  &    \\\hline
   \end{tabular}\end{center}\label{table:grid}  
\end{table}

From Tables~\ref{table:grid}, we observe that our new method of grid neighbor search
successfully infers other solutions than the chemical graphs $\C^\dagger$
 inferred by the standard Stage~4
even though Stage~5 could not find many chemical isomers $\C^*$ of $\C^\dagger$.
The branch-and-bound method for solving an MILP sometimes takes
an extremely large execution time for the same size of instances. 
We introduce a time limit to bound an entire running time to skip such instances
during an execution of testing the feasibility of grids in the neighbor $N(r)$.
From Tables~\ref{table:grid}, we see that at least around a half number of grids in $N(r)$
were feasible and provided new solutions.   
 
 
